A Temporal Module for Logical Frameworks

In artificial intelligence, multi agent systems constitute an interesting typology of society modeling, and have in this regard vast fields of application, which extend to the human sciences. Logic is often used to model such kind of systems as it is easier to verify than other approaches, and provides explainability and potential validation. In this paper we define a time module suitable to add time to many logic representations of agents.

==> eptcsdata.tex <==
\providecommand{\firstpage}{340}
\providecommand{\publicationstatus}{B. Bogaerts, E. Erdem, P. Fodor, A. Formisano,\\ 
G. Ianni, D. Inclezan, G. Vidal, A. Villanueva, \\
M. De Vos, F. Yang (Eds.): International \\
Conference on Logic Programming 2019 (ICLP'19).\\
EPTCS 306, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.306.40}{10.4204/EPTCS.306.40}}

